Phase function methods for second order inhomogeneous linear ordinary differential equations

It is well known that second order homogeneous linear ordinary differential equations with slowly varying coefficients admit slowly varying phase functions. This observation underlies the Liouville-Green method and many other techniques for the asymptotic approximation of the solutions of such equations. It is also the basis of a recently developed numerical algorithm that, in many cases of interest, runs in time independent of the magnitude of the equation's coefficients and achieves accuracy on par with that predicted by its condition number. Here we point out that a large class of second order inhomogeneous linear ordinary differential equations can be efficiently and accurately solved by combining phase function methods for second order homogeneous linear ordinary differential equations with a variant of the adaptive Levin method for evaluating oscillatory integrals.

==> algorithm.tex <==
\begin{section}{Numerical algorithm}
\label{section:algorithm}

\begin{subsection}{An adaptive spectral for ordinary differential equations}
\label{section:algorithm:odesolver}
\end{subsection}

\end{section}


==> figures.tex <==
\begin{figure}[h!]
\centering
\hfil
\includegraphics[width=.60\textwidth]{airyplot1-err.pdf}
\hskip 3em
\hfil

\hfil
\includegraphics[width=.40\textwidth]{airyplot1-time.pdf}
\hfil 
\includegraphics[width=.40\textwidth]{airyplot2-time.pdf}
\hfil

\hfil
\includegraphics[width=.40\textwidth]{airyplot1-coefs.pdf}
\hfil
\includegraphics[width=.40\textwidth]{airyplot2-coefs.pdf}
\hfil

\caption{
The results of the first set of experiments of Subsection~\ref{section:experiments:airy}.
The plot on the first rwo gives the maximum observed absolute errors in the solutions
obtained by the phase function method and the conventional solver as functions of $\lambda$.
The plot on the left-hand side of the second row gives the time required by the phase method as
a function of $\lambda$, while the plot on the right-hand side of the second row gives the time
required by the conventional solver as a function of $\lambda$.
The plot on the left-hand side of the third row gives the number of coefficients
in the piecewise Chebyshev expansions of the phase function and the Levin solution
as functions of $\lambda$, whereas the plot on the right-hand side of the third row
gives the number of coefficients in the piecewise Chebyshev expansion
of the solution of (\ref{experiment:airy:ivp}) produced by the conventional solver.
}
\label{figure:airyplots1}
\end{figure}

\vfil\eject
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vfil
\begin{figure}

\centering
\hfil
\includegraphics[width=.40\textwidth]{airyplot3-err.pdf}
\hfil
\includegraphics[width=.40\textwidth]{airyplot3-time.pdf}
\hfil

\hfil
\includegraphics[width=.40\textwidth]{airyplot3-coefs1.pdf}
\hfil
\includegraphics[width=.40\textwidth]{airyplot3-coefs2.pdf}
\hfil


\caption{
The results of the second set of experiments of Subsection~\ref{section:experiments:airy},
which demonstrate the behavior of our algorithm for values of the parameter $\lambda$
between $1$ and $200$.
The plots in the first row compare the running time and accuracy
of the phase method with a conventional solver.  The plot in the lower left
give the number of Chebyshev coefficients used to represent the phase function
and the Levin solution, while the plot in the lower right gives the number of 
Chebyshev coefficients used to represent the solution produced by the conventional
solver.  
}
\label{figure:airyplots2}
\end{figure}
\vfil

\vfil\eject
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vfil
\begin{figure}[h!]
\centering
\hfil
\includegraphics[width=.40\textwidth]{airyplot4-err.pdf}
\hfil
\includegraphics[width=.40\textwidth]{airyplot4-time.pdf}
\hfil

\hfil
\includegraphics[width=.40\textwidth]{airyplot4-coefs1.pdf}
\hfil
\includegraphics[width=.40\textwidth]{airyplot4-coefs2.pdf}
\hfil

\caption{
The results of the third set of experiments of Subsection~\ref{section:experiments:airy},
which demonstrate the behavior of our algorithm for values of the parameter $\lambda$
between $1$ and $10$.
The plots in the first row compare the running time and accuracy
of the phase method with a conventional solver.  The plot in the lower left
give the number of Chebyshev coefficients used to represent the phase function
and the Levin solution, while the plot in the lower right gives the number of 
Chebyshev coefficients used to represent the solution produced by the conventional
solver.  
}
\label{figure:airyplots3}
\end{figure}
\vfil


\vfil\eject
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\vfil
\begin{figure}[h!]
\centering

%% \hfil
%% \includegraphics[width=.32\textwidth]{exp2plot-err.pdf}
%% \hfil
%% \includegraphics[width=.32\textwidth]{explot2-time.pdf}
%% \hfil
%% \includegraphics[width=.32\textwidth]{explot2-coefs.pdf}
% \hfil

\caption{The results of the experiments of Subsection\ref{section:experiments:two}
}
\label{figure:exp2plots}
\end{figure}
\vfil


==> junk <==
%% \begin{equation*}
%% %% D_{ij} = 
%% %% \begin{cases}
%% %% \frac{c_i (-1)^{i+j}}{c_j(x_i-x_j)} & i \neq j \\
%% %% -\sum_{l\neq i} D_{il} & i = j,
%% %% \end{cases}
%% \renewcommand*{\arraystretch}{2}
%% \small
%% B =
%% \frac{2}{b_0-a_0}
%% \left(
%% \begin{array}{ccccccc}
%% \frac{1}{6} \left(1+2(k-1)^2\right) & - 2 \frac{1}{1-x_1} & 2 \frac{1}{1-x_2} & \cdots & 2 \frac{(-1)^{k-2}}{1-x_{k-2}} & \frac{1}{2} (-1)^{k-1}\\
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \frac{1}{2}  \frac{1}{1-x_1} & -\frac{1}{2} \frac{x_1}{1-x_1^2} &  - \frac{1}{x_1-x_2} & \cdots &\frac{(-1)^{k-3}}{x_1-x_{k-2}}&
%%  \frac{1}{2} \frac{(-1)^{k-2}}{1+x_1}\\
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% -\frac{1}{2}  \frac{1}{1-x_2} & -\frac{1}{x_2-x_1} &  - \frac{1}{2}\frac{x_2}{1-x_2^2} & \cdots & \frac{(-1)^{k-4}}{x_2-x_{k-3}}&
%%  \frac{1}{2} \frac{(-1)^{k-3}}{1+x_2}\\
%% \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% -\frac{1}{2}  \frac{(-1)^{k-2}}{1-x_{k-2}} & \frac{(-1)^{k-3}}{x_{k-2}-x_1} &  \frac{(-1)^{k-4}}{x_{k-2}-x_2} & \cdots & -\frac{1}{2} \frac{y_{k-2}}{1-x_{k-2}^2}&
%%  -\frac{1}{2} \frac{1}{1+x_{k-2}}\\
%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% -\frac{1}{2} (-1)^{k-1} & -2\frac{(-1)^{k-2}}{1+x_1} &  -2\frac{(-1)^{k-3}}{1+x_2} & \cdots & 2 \frac{1}{1+x_{k-2}}&
%%  -\frac{1}{6} (1+2(k-1)^2)
%% \end{array}
%% \right)
%% \end{equation*}
%% %
%% and the entries of the diagonal matrix
%% come from the vector (\ref{algorithm:vector}).
%% %
%% Since the slowly varying solution $p_0$ whose existence is established in \cite{Levin}
%% solves  $D\left[p_0\right](t) = f(t)$, it follows that the obtained solution must
%% closely approximate $p_0$.  

%% It can be easily verified that if  $p$ satisfies
%% %
%% \begin{equation}
%% p'(t) + g'(t) p(t) = f(t), \ \ \ \ \ a < t < b,
%% \label{levin:ode}
%% \end{equation}
%% %
%% then 
%% %
%% \begin{equation}
%% \frac{d}{dt} \left( \exp\left(g(t) \right) p(t)  \right) = \exp(g(t)) f(t).
%% \end{equation}
%% %
%% It follows that
%% %
%% \begin{equation}
%% \int_a^b \exp(g(t)) f(t)\ dt = p(b) \exp(g(b)) - p(a) \exp(g(a))
%% \end{equation}
%% %
%% whenever $p$ is a solution of (\ref{levin:ode}).  

%% In \cite{Levin}, it was observed that when $f$ and $g$ are slowly varying
%% functions and $g$ , (\ref{levin:ode}) admits slowly varying solutions.  

%% Under the change of variables
%% %
%% \begin{equation}
%% x = g(t), 
%% \end{equation}
%% %

%% %

%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \begin{subsection}{The classical Levin method}
%% The Levin method is a classical technique for evaluating integrals of the form
%% %
%% \begin{equation}
%% \int_a^b \exp(g(t)) f(t)\ dt.
%% \label{levin:int}
%% \end{equation}
%% %
%% It operates by solving the ordinary differential equation
%% %
%% \begin{equation}
%% p'(t) + g'(t) p(t) = f(t)
%% \label{levin:eq}
%% \end{equation}
%% %
%% in order to construct a function $p$ such that
%% %
%% \begin{equation}
%% \frac{d}{dt} \left( \exp(g(t)) p(t) \right) = \exp(g(t)) f(t).
%% \label{levin:der}
%% \end{equation}
%% %
%% The value of the integral (\ref{levin:int}) is then equal to
%% %
%% \begin{equation}
%% p(b) \exp(g(b)) - p(a) \exp(g(a)).
%% \end{equation}
%% %

%% It is shown in \cite{Levin} that when $g$ is of large magnitude but $g$ and $f$ are slowly varying
%% functions, the Levin method is much more efficient than standard techniques for evaluating 
%% (\ref{levin:int}).   
%% When  $g(t) =  \lambda^2 u(t)$ with $u$ invertible on $[a,b]$  this can
%% be easily seen by  introduce the new variable
%% $x=u^{-1}(t)$.  This transforms (\ref{levin:eq}) into 
%% %
%% \begin{equation}
%% p'(x) + \lambda^2 p(x) = \frac{f\left(u^{-1}(x)\right)}{u'\left(u^{-1}(x)\right)}.
%% \label{levin:eq2}
%% \end{equation}
%% %
%% %
%% If
%% %
%% \begin{equation}
%%  \frac{f\left(u^{-1}(x)\right)}{u'\left(u^{-1}(x)\right)}
%% = \int_{-\infty}^\infty F(\xi) \exp(i\xi x)\ dx,
%% \end{equation}
%% %
%% then
%% %
%% \begin{equation}
%% p_0(x) = 
%%  \frac{f\left(u^{-1}(x)\right)}{u'\left(u^{-1}(x)\right)}
%% = \mbox{PV}\  \int_{-\infty}^\infty \frac{F(\xi)}{i(\xi+\lambda^2)}
%%  \exp(i\xi x)\ dx,
%% \end{equation}
%% %
%% solves (\ref{levin:eq})


%% In \cite{Levin}, it was shown that
%% If 
%% %
%% \begin{equation}
%% \end{equation}
%% %
%% then
%% %
%% \begin{equation}
%% %% p_0(x) = \mbox{PV} \int \frac{F(\xi)}{\xi+
%% \end{equation}
%% %
%% is a solution of ().  This ``Levin solution'' is 

%% Clearly, the differential operator
%% %
%% %
%% has a one-dimensional nullspace consisting of the span of the function
%% %
%% \begin{equation}
%% \eta(t) = \exp(-g(x)).
%% \end{equation}
%% %
%% When () is discretized using a Chebyshev spectral collocation method which
%% is the resulting linear system is solved using, the 
%% %
%% %

%% \begin{equation}
%% p(x) = p_0(x) - \left< p_0, \eta\right> \eta
%% \end{equation}

%% \end{subsection}

%% Equation (\ref{phase:kummer}) is known  as Kummer's equation after E.E.~Kummer who studied it in \cite{Kummer}.



%% It is easy to verify that if $\alpha$ is a phase function
%% for (\ref{introduction:hom}) then $\alpha'$ satisfies
%% the second order nonlinear differential equation
%% %
%% %
%% and


%% If $y(t) = \exp(r(t))$ satisfies the second order differential equation
%% %
%% \begin{equation}
%% y''(t) + q(t) y(t) = 0, \ \ \ \ \ a < t < b,
%% \label{phase:ode}
%% \end{equation}
%% %
%% then it can be easily seen that r(t) solves the Riccati equation
%% %
%% \begin{equation}
%% r''(t) + (r'(t))^2 + q(t) = 0,\ \ \ \ \ a < t <  b.
%% \label{phase:riccati}
%% \end{equation}
%% %
%% Letting  $r(t) = i \alpha(t) + \beta(t)$  yields the system
%% of ordinary differential equations
%% %
%% \begin{equation}
%% \left\{
%% \begin{aligned}
%% q(t) - (\alpha'(t))^2 + (\beta'(t))^2+ \beta''(t)  &=0 \\
%%  2 \alpha'(t) \beta'(t) + \alpha''(t) &= 0.
%% \end{aligned}
%% \right.
%% \label{phase:system}
%% \end{equation}
%% %
%% The second of these can be rearranged as 
%% %
%% \begin{equation}
%% \beta'(t) = -\frac{1}{2} \frac{\alpha''(t)}{\alpha'(t)},
%% \label{phase:beta}
%% \end{equation}
%% %
%% and when this expression is inserted into the first equation in (\ref{phase:system}) 
%% we arrive at 
%% %
%% \begin{equation}
%% q(t) - (\alpha'(t))^2  + \frac{3}{4} \left(\frac{\alpha''(t)}{\alpha'(t)}\right)^2
%% - \frac{\alpha'''(t)}{2\alpha'(t)} = 0,\ \ \ \ \ a <t <b.
%% \label{phase:kummer}
%% \end{equation}
%% %
%% It is clear  that if  $\alpha$ does not vanish on $(a,b)$ and satisfies (\ref{phase:kummer})
%% there, then
%% %
%% \begin{equation}
%% r(t) = i \alpha(t) -\frac{1}{2} \log\left(\alpha'(t)\right),
%% \label{phase:rsol}
%% \end{equation}
%% %
%% where the implicit constant of integration and the choice of branch cut for
%% the logarithm are irrelevant,
%% is a solution of the Riccati equation (\ref{phase:riccati}) and 
%% %
%% \begin{equation}
%% \frac{\exp(i \alpha(t))}{\sqrt{\alpha'(t)}}
%% =
%% \frac{\cos( \alpha(t))}{\sqrt{\alpha'(t)}}
%% + i \frac{\sin( \alpha(t))}{\sqrt{\alpha'(t)}}
%% \end{equation}
%% %
%% is a solution of the original ordinary differential equation (\ref{phase:ode}).

%% Equation~(\ref{phase:kummer}) is known as Kummer's equation, after E.~E.~Kummer who
%% considered it in \cite{Kummer} and we  refer to its solutions 
%%  as phase functions for the ordinary differential equation (\ref{phase:ode}).
%% When the coefficients $p$ and $q$ are real-valued,
%%  $\alpha(t)$ is also real-valued, and the functions
%% %
%% \begin{equation}
%% u(t) = \frac{\cos( \alpha(t))}{\sqrt{\alpha'(t)}}
%% \ \ \mbox{and} \ \ \ 
%% v(t) = \frac{\sin( \alpha(t))}{\sqrt{\alpha'(t)}}
%% \label{phase:basis}
%% \end{equation}
%% %
%% are linearly independent real-valued solutions of (\ref{phase:ode}) which form a basis in its 
%% space of solutions.   


%% If $\alpha$ is a phase function and $u$ and $v$
%% are as in (\ref{phase:basis}), then a straightforward 
%% computation shows that the modulus function
%% %
%% \begin{equation}
%% m(t) = (u(t))^2 + (v(t))^2 = \frac{\omega(t)}{\alpha'(t)}
%% \end{equation}
%% %
%% satisfies the differential equation
%% %
%% \begin{equation}
%% m'''(t) + 3p(t) m''(t) + (2 (p(t))^2 + p'(t) + 4 q(t))m'(t) +
%% (4p(t)q(t) + 2q'(t) ) m(t) = 0.
%% \label{phase:appell}
%% \end{equation}
%% %
%% %% In fact, the solutions of (\ref{phase:appell}) are the linear combinations of 
%% %% products of the solutions of (\ref{phase:ode}).
%% We refer to (\ref{phase:appell}) as Appell's equation in light of the article
%% \cite{Appell}.  

%% Given any pair $u, v$  of solutions of (\ref{phase:ode}) whose Wronskian $\omega(t)$
%% and the associated modulus function $m(t) = (u(t))^2 + (v(t))^2$ are
%% nonzero on $(a,b)$,  it can be shown by a straightforward calculation that
%% %
%% \begin{equation}
%% \alpha'(t) = \frac{\omega(t)}{(u(t))^2+(v(t))^2}
%% \label{phase:alphap}
%% \end{equation}
%% %
%% satisfies (\ref{phase:kummer}) on that interval.  It follows that any antiderivative of $\alpha'$ 
%% is a phase function for (\ref{phase:ode}) on $(a,b)$.  
%% Requiring that (\ref{phase:basis}) holds
%% determines $\alpha$  up to an additive constant which is an integral multiple of $2\pi$, but further restrictions
%% are required to determine it uniquely.
%% We will nonetheless, by a slight abuse of terminology, refer to  ``the phase function generated
%% by the pair of solutions $u,v$''  with the understanding that the choice of constant
%% is of no consequence.

%% %% \end{subsection}
%% %% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%% %% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% %% \begin{subsection}{Reduction to normal form}
%% %% \label{section:phase:normal}

%% %% If $y$ solves (\ref{phase:ode}), then
%% %% %
%% %% \begin{equation}
%% %% \tilde{y}(t) = \exp\left(-\frac{1}{2} \int p(t)\ dt \right) y(t) 
%% %% \label{phase:transform}
%% %% \end{equation}
%% %% %
%% %% satisfies
%% %% %
%% %% \begin{equation}
%% %% \tilde{y}''(t) +  \tilde{q}(t) \tilde{y}(t) = 0, \ \ a < t < b,
%% %% \label{phase:normal}
%% %% \end{equation}
%% %% %
%% %% where
%% %% %
%% %% \begin{equation}
%% %% \tilde{q}(t) = q(t) - \frac{p(t)}{2} - \frac{(p(t))^2}{4}.
%% %% \label{phase:qtilde}
%% %% \end{equation}
%% %% %
%% %% Equation~(\ref{phase:normal}) is often called the normal form of (\ref{phase:ode}).
%% %% The effects of this transformation on the various formulas discussed above
%% %% are easy to discern.  In particular, Riccati's equation becomes
%% %% %
%% %% \begin{equation}
%% %% \tilde{r}''(t) + (\tilde{r}'(t))^2 + \tilde{q}(t) = 0,
%% %% \label{phase:norm_riccati}
%% %% \end{equation}
%% %% %
%% %% Kummer's equation now takes the form
%% %% %
%% %% \begin{equation}
%% %% \tilde{q}(t) - (\tilde{\alpha}'(t))^2 + \frac{3}{4} \left(\frac{\tilde{\alpha}''(t)}
%% %% {\tilde{\alpha}'(t)}\right)^2
%% %% - \frac{\tilde{\alpha}'''(t)}{2\tilde{\alpha}'(t)} = 0,\ \ a <t <b,
%% %% \label{phase:norm_kummer}
%% %% \end{equation}

%% %% Appell's equation becomes
%% %% %
%% %% \begin{equation}
%% %% \tilde{m}'''(t)  + 4 \tilde{q}(t) \tilde{m}'(t) + 2 \tilde{q}'(t) \tilde{m}(t) = 0,
%% %% \end{equation}
%% %% %
%% %% and it is the functions
%% %% %
%% %% \begin{equation}
%% %% \tilde{u}(t) = \frac{\cos(\tilde{\alpha}(t))}{\sqrt{\tilde{\alpha}'(t)}}
%% %% \ \ \mbox{and} \ \ \ 
%% %% \tilde{v}(t) = \frac{\sin(\tilde{\alpha}(t))}{\sqrt{\tilde{\alpha}'(t)}}
%% %% \label{phase:norm_sols}
%% %% \end{equation}
%% %% %
%% %% which form a  basis in the space of solutions of (\ref{phase:normal}).

%% %% We observe that when (\ref{phase:qtilde}) is inserted into (\ref{phase:norm_kummer})
%% %% it simply becomes (\ref{phase:kummer}), so that Kummer's equation is unchanged
%% %% by this transformation.  Similarly, (\ref{phase:alphap}) is invariant 
%% %% under  (\ref{phase:transform}), which implies that
%% %% %
%% %% \begin{equation}
%% %% \alpha'(t) = \tilde{\alpha}'(t).
%% %% \end{equation}
%% %% %
%% %% So while the solution of Riccati's equation and the basis functions are modified
%% %% by the transformation (\ref{phase:transform}), the phase function $\alpha$ is invariant.  
%% %% It does not matter, then, whether the form (\ref{phase:ode}) or its normal form (\ref{phase:normal})
%% %% is considered.   Either set of solutions (\ref{phase:basis}) or (\ref{phase:norm_sols}) 
%% %% can be recovered once $\alpha$ has been calculated.
%% %% %% Accordingly, we will always consider ordinary differential equations in normal form
%% %% %% throughout the remainder of this article.

%% %% \end{subsection}

%% \begin{remark}
%% {\bf Remark about general form}
%% \end{remark}


%% %% When standard solvers for ordinary differential
%% %% equations are used in this case, their running times grow with the magnitude of $q$.
%% %% Asymptotic methods;
%% %% but, in many cases of interest, they are unable to obtain accuracy on par with
%% %% the condition number of the problem (\ref{introduction:ode}).

%%  Under mild conditions on $q$, 
%% By constrast, under mild conditions of $q$, the algorithm of \cite{BremerKummer}
%% obtains accuracy on par with that predicted by the condition number
%% of (\ref{introduction:ode})  in time which is independent of the 
%% In fact, bounds on the complexity of the phase  function $\alpha$ constructed by the 
%% algorithm of \cite{BremerKummer} under mild conditions on the coefficient $q$ are established in a companion paper
%% \cite{BremerRokhlin}.

%% %% is independent of the 
%% %% numerically constructs a phase function $\alpha$  such that
%% %% %
%% %% %
%% %% form a basis in the space of solutions of  (\ref{introduction:hom}).
%% %% When $q$ is of large magnitude, the solutions of (\ref{introduction:hom})
%% %% are highly oscillatory, but, assuming $q$ is nonoscillatory, the phase
%% %% function $\alpha$ is nonoscillatory.  
%% %% Bounds on the 
%% In many cases of interest, it runs in time independent
%% of the magnitude of the coefficients and achieves accuracy on par with that predicted by 
%% the condition number of  the problem.  The algorithm of \cite{BremerKummer}
%% is extended to the case of equations of the form (\ref{introduction:hom})
%% which have turning points in \cite{bremerphase}.  It is also observed there that slowly
%% varying phase functions
%% extend across turing points of odd orders but not turning points of even orders.
%% {\bf more here.}


%% Since  the frequency of  their oscillations increases with the magnitude of $q$,
%% when standard ODEs solvers are applied to (\ref{introduction:hom}), 
%% their running times grow  with the magnitude of $q$.  
%% By contrast,  the running time of the 
%% algorithm of \cite{BremerKummer}  is independent of the magnitude of $q$.

%% %

%
%% admits a slowly varying phase function.  
%% That is, there exists a slowly 
%% varying $\alpha$ such that 
%% %
%% %
%% form a basis in the space of solutions of (\ref{introduction:hom}).
It is also the basis of the 

The article \cite{BremerRokhlin} presents a theorem which bounds the complexity of a phase function 
$\alpha$ such that
%
%
for 
(\ref{introduction:hom}) in the case in which  its solutions are purely oscillatory.
An efficient numerical algorithm for constructing nonoscillatory phase functions in this
case is presented in  \cite{BremerKummer}. 
